Double brane holographic model dual to 2d ICFTs

A minimal single-brane holographic model can be used as a dual to 2d conformal interfaces (ICFTs) to calculate the transmission coefficient $\mathcal{T}$ of energy transported across the defect as well as boundary entropy $\log g$, the additional entanglement entropy for some sub-region that encloses the defect. Both $\mathcal{T}$ and $\log g$ are uniquely determined by the tension characterizing the brane. In contrast, in field theory defects typically the transmission coefficient can be dialed from 0 to 1 independently for each allowed value of $\log g$. To address this discrepancy, we look at a double brane (3-region bulk) holographic model. Merger of two single brane interfaces creates genuinely new interfaces which indeed allow a range of accessible transmission coefficients for a fixed value of $\log g$. In particular, the $\mathcal{T}=0$ limit of two completely decoupled BCFTs can be achieved.

==> v2 /3RegionHolographicDiagram.tex <==
\begin{figure}[ht!]
\centering
\begin{tikzpicture}[scale=0.50]

% Horizontal line at top of 3 non-zero regions
\draw[<-,blue,thick] (-7.5,3) to (-4.5,3);
\draw[-,blue,thick] (-1.5,3) to (1.5,3);
\draw[->,blue,thick] (4.5,3) to (7.5,3);

% Vertical lines representing branes
\draw[-,blue,thick] (-4.5,3) to (-3.5,0);
\draw[-,blue,thick] (-2.5,0) to (-1.5,3);
\draw[-,blue,thick] (1.5,3) to (2.5,0);
\draw[-,blue,thick] (3.5,0) to (4.5,3);

% Co-ordinate lines (left, then right)
\draw[->,red!30!blue!90!, very thick] (-4.5,3) -- (-4.5,1);
\node[red!30!blue!90!] at (-5,1.5) {$y_{L}$};
\draw[->,red!30!blue!90!, very thick] (-4.5,3) -- (-3,3);
\node[red!30!blue!90!] at (-3.5,3.5) {$u_{L}$};

\draw[->,red!30!blue!90!, very thick] (4.5,3) -- (4.5,1);
\node[red!30!blue!90!] at (5,1.5) {$y_{R}$};
\draw[->,red!30!blue!90!, very thick] (4.5,3) -- (6,3);
\node[red!30!blue!90!] at (5.5,3.5) {$u_{R}$};

% marking central region
\draw[<->,thin] (-1.5,0.5) to (1.5,0.5);
\node at (0,1) {$\delta$};

% Central region goes to single point at the boundary
\draw[->,thin] (0,-0.5) to (0,-2);
\node at (1.5,-1.5) {$\delta=0$};

% 3region model (left top, then brane, then angle)
\node[blue!70!] at (-9,-11) {$M_{L}$};
\node[red!70!] at (-9,-12) {$l_{L}$};

\draw[-,blue,very thick] (-10,-4) to (-6,-4) to (-7,-8) to (-11,-8) ;
\draw[->,red!50!blue!70!, thick, style={decorate, decoration={snake, post=lineto ,post length=0.1cm}}] (-10,-7.5) -- (-8,-6.5);
\node[red!50!blue!70!] at (-10.5,-7) {$I$};
\draw[->,red!50!blue!70!, thick, style={decorate, decoration={snake, post=lineto ,post length=0.1cm}}] (-8,-5.5) -- (-10,-4.5);
\node[red!50!blue!70!] at (-7.5,-5) {$R$};

\draw[-,blue, very thick, fill=red!10!, style={decoration=snake}] (-4,-9) -- (-6,-4) -- (-7,-8) -- (-5,-13) decorate{-- (-4,-9)};
\node[red!70!] at (-4,-13) {$\sigma_{1}$};

\draw[dashed, blue, thin] (-7,-8) to (-7,-11);
\draw[->, red, thick] (-7,-9.5) arc(-90:-68.2:1.5cm);
\node[red!70!] at (-6.5,-10) {$\theta_{L}$};

% 3region model (right top, then brane, then angle)
\node[blue!70!] at (9,-11) {$M_{R}$};
\node[red!70!] at (9,-12) {$l_{R}$};

\draw[-,blue,very thick] (10,-4) to (6,-4) to (7,-8) to (11,-8);
\draw[->,red!50!blue!70!, thick, style={decorate, decoration={snake, post=lineto ,post length=0.1cm}}] (7,-6) -- (9,-5);
\node[red!50!blue!70!] at (7.5,-5) {$T$};

\draw[-,blue, very thick, fill=green!10, style={decoration=snake}] (4,-9) -- (6,-4) -- (7,-8) -- (5,-13) decorate{-- (4,-9)};
\node[red!70!] at (4,-13) {$\sigma_{2}$};

\draw[dashed, blue, thin] (7,-8) to (7,-11);
\draw[->, red, thick] (7,-9.5) arc(-90:-112.8:1.5cm);
\node[red!70!] at (6.6,-10) {$\theta_{R}$};

% 3region model (centre, then left brane, then right brane, then angles )
\node[blue!70!] at (0,-12) {$M_{C}$};
\node[red!70!] at (0,-13) {$l_{C}$};

\draw[-,blue,very thick, fill=red!10!, style={decoration=snake}] (0,-4) -- (-3,-9) decorate{-- (-3,-13)} -- (0,-8) -- (0,-4);

\draw[-,blue,very thick, fill=green!10!, style={decoration=snake}] (0,-4) -- (3,-9) decorate{-- (3,-13)} -- (0,-8) -- (0,-4);

\draw[dashed, blue, thin] (0,-8) to (0,-11);
\draw[->, red, thick] (0,-9.5) arc(-90:-121:1.5cm);
\node[red!70!] at (-0.5,-10) {$\theta_{CL}$};
\draw[->, red, thick] (0,-10) arc(-90:-59:2cm);
\node[red!70!] at (0.8,-10.5) {$\theta_{CR}$};



\end{tikzpicture}
\caption{\label{fig1}The 3 region holographic model representing the fusion of two defects. I is the gravitational wave scattered from the left, and R and T are the reflected and transmitted waves on the left and right of the interface respectively.}
\end{figure}
